Convolutional Hypercomplex Embeddings for Link Prediction

Knowledge graph embedding research has mainly focused on the two smallest normed division algebras, $\mathbb{R}$ and $\mathbb{C}$. Recent results suggest that trilinear products of quaternion-valued embeddings can be a more effective means to tackle link prediction. In addition, models based on convolutions on real-valued embeddings often yield state-of-the-art results for link prediction. In this paper, we investigate a composition of convolution operations with hypercomplex multiplications. We propose the four approaches QMult, OMult, ConvQ and ConvO to tackle the link prediction problem. QMult and OMult can be considered as quaternion and octonion extensions of previous state-of-the-art approaches, including DistMult and ComplEx. ConvQ and ConvO build upon QMult and OMult by including convolution operations in a way inspired by the residual learning framework. We evaluated our approaches on seven link prediction datasets including WN18RR, FB15K-237 and YAGO3-10. Experimental results suggest that the benefits of learning hypercomplex-valued vector representations become more apparent as the size and complexity of the knowledge graph grows. ConvO outperforms state-of-the-art approaches on FB15K-237 in MRR, Hit@1 and Hit@3, while QMult, OMult, ConvQ and ConvO outperform state-of-the-approaches on YAGO3-10 in all metrics. Results also suggest that link prediction performances can be further improved via prediction averaging. To foster reproducible research, we provide an open-source implementation of approaches, including training and evaluation scripts as well as pretrained models.

==> figures/YAGO3_10-per-relation.tex <==
\begin{table*}[tb]
\caption{MRR link prediction results per relations on YAGO3-10.}
\label{table:mrr_per_rel_yago3}
\centering
\scalebox{0.80}{%
\begin{tabular}{@{}lcccccccc}
\toprule
\textbf{Relation}    & train freq.                 & test freq.                  &\textbf{\baseapproach}& \textbf{\baseapproachocto}& \textbf{\approach} & \textbf{\approachocto}\\ \midrule
% playsFor             &                            &                             &\textbf{.639}          & .634                         & \underline{.635}   &  .575              \\
hasOfficialLanguage  &                            &                             &.562                   & \textbf{.646}                & .557               & \underline{.566}  \\
isAffiliatedTo       &                            &                             &  \textbf{.732}          & .701                         & \underline{.704}   & .615              \\
% isInterestedIn       &                            &                             &  .642                   & \textbf{.775}                & .431               & .687              \\
diedIn               &                            &                             &  .169                   & .172                         & .171               & \textbf{.174}     \\
hasGender            &                            &                             &  \textbf{.489}          & .485                         & .475               & .481              \\
isLocatedIn          &                            &                             &  .338                   & \textbf{.343}                & .328               & \textbf{.343}      \\
%hasMusicalRole       &                            &                             &  \textbf{.307}          & \underline{.262}             & .227               & .214              \\
%actedIn              &                            &                             &  \textbf{.121}          & \textbf{.127}                & .117               & .113              \\
%wasBornIn            &                            &                             &  .186                   & \textbf{.188}                & .137               & .129              \\
h%appenedIn           &                            &                             &  \textbf{.545}          & .500                         & .467               & .412              \\
hasChild             &                            &                             &  \textbf{.198}          & .175                         & \underline{.192}   & .159              \\
influences           &                            &                             &  .101                   & .106                         & \textbf{.133}      & .102              \\
participatedIn       &                            &                             &  .350                   & \underline{.382}             & \textbf{.406}      & .371              \\
wroteMusicFor        &                            &                             &  .239                   & .232                         & \textbf{.244}      & .204              \\
directed             &                            &                             &  .525                   & \textbf{.538}                & .508               & .471              \\
hasWonPrize          &                            &                             &  \underline{.279}       & .278                         & \textbf{.285}      & .272              \\
created              &                            &                             &  \underline{.331}       & .325                         & .317               & \textbf{.334}     \\
%edited               &                            &                             &  \textbf{.225}          & \underline{.222}             & .181               & .196              \\
%isConnectedTo        &                            &                             &  \underline{.481}       & .436                         & \textbf{.482}      & .411              \\
%dealsWith            &                            &                             &  \underline{.375}       & \textbf{.467}                & .329               & .268              \\
%livesIn              &                            &                             &  .147                   & \textbf{.237}                & .171               & .179              \\
isMarriedTo          &                            &                             &  \textbf{.985}          & \textbf{.985}                & \textbf{.985}      & \textbf{.985}     \\
worksAt              &                            &                             &  \textbf{.421}          & .398                         & \underline{.403}   & .319              \\
isPoliticianOf       &                            &                             &  .411                   & .492                         & \textbf{.567}      & .503              \\
isCitizenOf          &                            &                             &  .293                   & .274                         & \textbf{.300}      & \underline{.297}  \\
graduatedFrom        &                            &                             &  \textbf{.177}          & .144                         & .111               & \underline{.149}  \\
isLeaderOf           &                            &                             &  .062                   & .08                          & .061               & \textbf{.096}     \\
hasCapital           &                            &                             &  .495                   & \textbf{.551}                & .514               & \underline{.517}  \\
exports              &                            &                             &  .082                   & \underline{.092}             & .084               & \textbf{.116}     \\
hasAcademicAdvisor   &                            &                             &  \textbf{.062}          & .041                         & .036               & \underline{.05}    \\
hasWebsite           &                            &                             &  .256                   & \underline{.502}             & .500               & \textbf{.511}     \\
owns                 &                            &                             &  .171                   & .209                         & .203               & \textbf{.416}     \\
hasNeighbor          &                            &                             &  \underline{.875}       & .542                         & \textbf{1.0}                & \underline{.875} \\
\bottomrule
\end{tabular}}
\end{table*}


==> figures/table-link-prediction-FB15K-237-per-relation.tex <==
\begin{table*}[tbp]
\caption{MRR link prediction performances for all \textit{person} related relations on FB15k-237.}
\label{table: mrr_per_rel_fb}
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
Relation Name                          &\baseapproach & \approach & \baseapproachocto &\approachocto \\ 
\midrule
people/person/nationality                     & .81           &.81      & .80               & \textbf{.83}     \\ 
people/person/gender                          & .93           & .88      & .93               & \textbf{.95}      \\ 
people/person/languages                       & .77           & .76      & .78               & \textbf{.81}     \\ 
people/person/profession                      & .61           & .57      & \textbf{.64}               & \textbf{.64}      \\
people/person/places\_lived                   & .21           & .12      & .19               & \textbf{.21}     \\
people/person/place\_of\_birth                & .19           & .12      & .19               & \textbf{.19}     \\
people/person/places\_lived                   & .21           & .12      & .19               & \textbf{.21}     \\ 
people/person/religion                        & .55           & .42      & .57               & \textbf{.58}     \\
people/person/spouse\_s                       & .97           & .94      & .97               & \textbf{.97}      \\
people/person/employment\_history             & .19           & .09      & \textbf{.23}              & .16      \\
\bottomrule
% people/ethnicity/geographic\_distribution     & .33           &  .28      & .29              & \textbf{.38}}      \\
% people/ethnicity/languages\_spoken            & .49           & .38       & .43              & \textbf{.52}}   \\

% country/capital                        & \textbf{.19}}           & .06      & .14               & .17      \\
% country/official\_language             & .52           & {\color{blue}\textbf{.65}}      & .59               &  {\color{blue}\textbf{.60}}      \\
% country/form\_of\_government           &  .62          & .75      & {\color{blue}\textbf{.82}}               & \textbf{.83}}      \\ 
% symptom/symptom\_of                     & .18           & {\color{blue}\textbf{.24}}      & .22               & \textbf{.27}}      \\
% disease/risk\_factors                   & .41           & .31      & \textbf{.50}}               & {\color{blue}\textbf{.48}}      \\
\end{tabular}
\end{table*}




==> figures/table-models.tex <==
\begin{table*}[tbp]
\centering
\caption{State-of-the-art \ac{KGE} models with their training strategies. $\emb{}$ denotes embeddings, $\overline{\emb{}} \in \ComplexNumbers$ corresponds to the complex conjugate of $\emb{.}$. $\ast$ denotes a convolution operation with $\omega$ kernel. $f$ denotes rectified linear unit function. $\bigstar,\otimes, \circ$ and $\cdot$ denote the Octonion, Quaternion, Hadamard and an inner product, respectively. $\triangleleft$ denotes unit normalization. $\ConvolutionWithProjection(\cdot,\cdot)$ corresponds to a convolution operation followed by linear transformation. The tensor product along the $n$-th mode is denoted by $\times_n$ and the core tensor is represented by $\mathcal{W}$. MSE, MR, BCE and CE denote mean squared error, margin ranking, binary cross entropy and cross entropy. NegSamp and AdvNegS.\ stand for negative sampling and adversarial negative sampling.}
  \label{table:models}
\scalebox{0.90}{%
\scriptsize
%\fontsize{8}{9.5}\selectfont
%\setlength{\tabcolsep}{1.3pt}
\begin{tabular}{@{}lccllll@{}}
  \toprule
  Model & Scoring Function-$\scoreFunc$ & Space & Loss & Training & Optimizer & Regularizer\\
  \midrule
   RESCAL~\cite{nickel2011three}          & $\emb{h}\cdot\mathcal{W}_r \cdot\emb{t}$                                                                       & $\RealNumbers$           & MSE & Full    & ALS     & L2 \\
   DistMult~\cite{yang2015embedding}      & $\langle \emb{h}, \emb{r}, \emb{t} \rangle$                                                                    & $\RealNumbers$    & MR  & NegSamp & Adagrad & Weighted L2 \\
   ComplEx~\cite{trouillon2016complex}    & $\real(\langle \emb{h}, \emb{r}, \overline{ \emb{t}} \rangle)$                                                 & $\ComplexNumbers$ & BCE & NegSamp & Adagrad & Weighted L2 \\
   ConvE~\cite{dettmers2018convolutional} & $f ( \vect ( f ([ \emb{h} ; \emb{r} ] \ast \omega )) \lt ) \cdot \emb{t}$                                      & $\RealNumbers$    & BCE & KvsAll  & Adam    & Dropout, BatchNorm \\
   TuckER~\cite{balavzevic2019tucker}     & $\mathcal{W} \times_1 \emb{h} \times_2 \emb{r} \times_3 \emb{t}$                                               & $\RealNumbers$    & BCE & KvsAll  & Adam    & Dropout, BatchNorm \\
   RotatE~\cite{sun2019rotate}            &  $-\parallel \emb{h} \circ \emb{r} - \emb{t}\parallel$                                                         & $\ComplexNumbers$
   &CE&AdvNegS. & Adam & --- \\                                                                     
   QuatE~\cite{zhang2019quaternion}       & $ \emb{h}\otimes \emb{r}^{\triangleleft} \cdot\emb{t}$                                                         & $\Quaternions$    & CE  & AdvNegS. & Adagrad    & Weighted L2 \\
%   QuaR~\cite{chen2020quaternion}       & $\parallel \emb{h} \circ \emb{r} - \emb{t}\parallel$                                                         & $\Quaternions$    & CE  &NegSamp & Adam   & - \\
%   OctonionE~\cite{zhang2019quaternion}   & $ \emb{h}\bigstar \emb{r}^{\triangleleft} \cdot\emb{t}$                                                        & $\Octonions$      & CE  & AdvNegSamp & Adagrad    & Weighted L2 \\
   \midrule
   \baseapproach (ours)                          & $ \emb{h} \otimes \emb{r} \cdot \emb{t}$                                                       & $\Quaternions$    & BCE & KvsAll  & Adam    & Dropout, BatchNorm \\
  \baseapproachocto (ours)                      & $\emb{h} \bigstar \emb{r} \cdot \emb{t}$                                                                       & $\Octonions$      & BCE & KvsAll  & Adam    & Dropout, BatchNorm\\
   \approach (ours)                              & $ \ConvolutionWithProjection(\emb{h},\emb{r} ) \circ (\emb{h} \otimes \emb{r}) \cdot \emb{t}$ & $\Quaternions$    & BCE & KvsAll  & Adam    & Dropout, BatchNorm \\
   %\midrule
   \approachocto (ours)                          & $\ConvolutionWithProjection(\emb{h},\emb{r} ) \circ (\emb{h} \bigstar \emb{r} ) \cdot \emb{t}$                 & $\Octonions$      & BCE & KvsAll  & Adam    & Dropout, BatchNorm\\
  \bottomrule
\end{tabular}}
\end{table*}
